Deuce: A Lightweight User Interface for Structured Editing

We present a structure-aware code editor, called Deuce, that is equipped with direct manipulation capabilities for invoking automated program transformations. Compared to traditional refactoring environments, Deuce employs a direct manipulation interface that is tightly integrated within a text-based editing workflow. In particular, Deuce draws (i) clickable widgets atop the source code that allow the user to structurally select the unstructured text for subexpressions and other relevant features, and (ii) a lightweight, interactive menu of potential transformations based on the current selections. We implement and evaluate our design with mostly standard transformations in the context of a small functional programming language. A controlled user study with 21 participants demonstrates that structural selection is preferred to a more traditional text-selection interface and may be faster overall once users gain experience with the tool. These results accord with Deuce's aim to provide human-friendly structural interactions on top of familiar text-based editing.

==> fig-sns-screenshot.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.25]{../oopsla-2017-deuce/images/sns-6-code-output.pdf}
\end{center}
\caption{Screenshot of \sns{} \snsNewVersion{}}
\label{fig:sns-screenshot}
\end{figure}


==> fig-transformations-1-names-only.tex <==
\begin{figure}[b]
%% \begin{figure}[t]
%% \small
\footnotesize

\begin{tabular}{ll}
\codeTool{Create Function from Definition} &
\codeTool{Rename Variable} \\
\codeTool{Create Function from Arguments} &
\codeTool{Introduce Local Variable(s)} \\
\codeTool{Create Function by Merging Definitions} &
\codeTool{Swap Variable Names and Usages} \\
\codeTool{Add Argument(s)} &
\codeTool{Swap Variable Usages} \\
\codeTool{Remove Argument(s)} &
\codeTool{Make Equal with Single Variable} \\
\codeTool{Reorder Argument(s)} &
\codeTool{Make Equal by Copying} \\
\codeTool{Move Definition(s)} &
\codeTool{Swap Expressions} \\
\codeTool{Swap Definition(s)} &
\codeTool{Reorder Expressions} \\
\codeTool{Inline Definition(s)} &
\codeTool{Make Single Line} \\
\codeTool{Duplicate Definition(s)} &
\codeTool{Make Multi-Line} \\
&
\codeTool{Align Expressions}
\end{tabular}

\caption{General-purpose transformations in \deuce{}.
\rkc{if user study section has a table of transformations used, then add all the
unused transformations there too, and get rid of this figure.}}
\label{fig:transformations-1-names-only}
\end{figure}

